Bayesian Optimisation for Robust Model Predictive Control under Model Parameter Uncertainty

We propose an adaptive optimisation approach for tuning stochastic model predictive control (MPC) hyper-parameters while jointly estimating probability distributions of the transition model parameters based on performance rewards. In particular, we develop a Bayesian optimisation (BO) algorithm with a heteroscedastic noise model to deal with varying noise across the MPC hyper-parameter and dynamics model parameter spaces. Typical homoscedastic noise models are unrealistic for tuning MPC since stochastic controllers are inherently noisy, and the level of noise is affected by their hyper-parameter settings. We evaluate the proposed optimisation algorithm in simulated control and robotics tasks where we jointly infer control and dynamics parameters. Experimental results demonstrate that our approach leads to higher cumulative rewards and more stable controllers.

==> sections/figure_scripts/mpc.tex <==
\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        
\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-0.65,xscale=0.8]
%uncomment if require: \path (0,184); %set diagram left start at 0, and has height of 184
%Rounded Rect [id:dp2929797119413593] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 233; green, 233; blue, 233 }  ,fill opacity=1 ][line width=1.5]  (9.38,41.41) .. controls (9.38,23.37) and (24,8.75) .. (42.04,8.75) -- (224.72,8.75) .. controls (242.76,8.75) and (257.38,23.37) .. (257.38,41.41) -- (257.38,139.39) .. controls (257.38,157.42) and (242.76,172.04) .. (224.72,172.04) -- (42.04,172.04) .. controls (24,172.04) and (9.38,157.42) .. (9.38,139.39) -- cycle ;
%Rounded Rect [id:dp052006627895683] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (69.79,121.88) .. controls (69.79,116.36) and (74.26,111.89) .. (79.78,111.89) -- (184.8,111.89) .. controls (190.32,111.89) and (194.79,116.36) .. (194.79,121.88) -- (194.79,151.85) .. controls (194.79,157.37) and (190.32,161.84) .. (184.8,161.84) -- (79.78,161.84) .. controls (74.26,161.84) and (69.79,157.37) .. (69.79,151.85) -- cycle ;
%Rounded Rect [id:dp05292973450874627] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (70.03,50.13) .. controls (70.03,43.51) and (75.39,38.14) .. (82.01,38.14) -- (182.8,38.14) .. controls (189.42,38.14) and (194.79,43.51) .. (194.79,50.13) -- (194.79,86.09) .. controls (194.79,92.71) and (189.42,98.08) .. (182.8,98.08) -- (82.01,98.08) .. controls (75.39,98.08) and (70.03,92.71) .. (70.03,86.09) -- cycle ;
%Curve Lines [id:da6174715136464386] 
\draw    (69.17,135.19) .. controls (42.92,116.66) and (41.4,101.24) .. (67.01,81.43) ;
\draw [shift={(69.03,79.89)}, rotate = 503.41] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da4801619241343944] 
\draw    (195.03,80.89) .. controls (221.62,102.22) and (220.66,114.43) .. (197.39,133.41) ;
\draw [shift={(195.17,135.19)}, rotate = 321.78] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Rounded Rect [id:dp7112132398300144] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]  (318.4,75.38) .. controls (318.4,67.98) and (324.4,61.98) .. (331.8,61.98) -- (400,61.98) .. controls (407.4,61.98) and (413.4,67.98) .. (413.4,75.38) -- (413.4,115.58) .. controls (413.4,122.98) and (407.4,128.98) .. (400,128.98) -- (331.8,128.98) .. controls (324.4,128.98) and (318.4,122.98) .. (318.4,115.58) -- cycle ;
%Straight Lines [id:da8873742018024069] 
\draw [line width=1.5]    (257.34,75.38) -- (314.4,75.38) ;
\draw [shift={(318.4,75.38)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Straight Lines [id:da3976171110066997] 
\draw [line width=1.5]    (261.54,118.38) -- (318.4,118.38) ;
\draw [shift={(257.54,118.38)}, rotate = 0] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;

% Text Node
\draw (133,143.68) node  [font=\normalsize]  {$s_{t+1} =f( s_{t} ,a_{t})$};
% Text Node
\draw (132.41,48.99) node  [font=\footnotesize] [align=left] {\textbf{{\small Optimization}}};
% Text Node
\draw (132.29,122.61) node  [font=\footnotesize] [align=left] {\textbf{{\small Transition Model}}};
% Text Node
\draw (234,107) node  [font=\footnotesize] [align=left] {Action};
% Text Node
\draw (32,107) node  [font=\footnotesize] [align=left] {State};
% Text Node
\draw (137,23.42) node   [align=left] {\textbf{{\small Model Predictive Control}}};
% Text Node
\draw (365.9,95.48) node   [align=left] {\textbf{{\small System}}};
% Text Node
\draw (290,63.16) node  [font=\small]  {$a^{*}_{t}$};
% Text Node
\draw (293,130.96) node  [font=\small]  {$s_{t+1}$};
% Text Node
\draw (128.41,66.11) node  [font=\footnotesize] [align=left] {
$\bullet \text{ Reward Function}$};
% Text Node
\draw (113.41,81.96) node  [font=\footnotesize]  {$\bullet \text{ Constraints}$};
\end{tikzpicture}

==> sections/figure_scripts/mpc_bo.tex <==
\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        
\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-0.75,xscale=0.95]
%uncomment if require: \path (0,727); %set diagram left start at 0, and has height of 727

%Rounded Rect [id:dp071734801571536] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]  (37.97,521.07) .. controls (37.97,511.76) and (45.52,504.21) .. (54.83,504.21) -- (281.11,504.21) .. controls (290.42,504.21) and (297.97,511.76) .. (297.97,521.07) -- (297.97,571.65) .. controls (297.97,580.96) and (290.42,588.51) .. (281.11,588.51) -- (54.83,588.51) .. controls (45.52,588.51) and (37.97,580.96) .. (37.97,571.65) -- cycle ;
%Rounded Rect [id:dp9922454977044957] 
\draw  [fill={rgb, 255:red, 233; green, 233; blue, 233 }  ,fill opacity=1 ][line width=1.5]  (4.27,397.59) .. controls (4.27,386.92) and (12.92,378.27) .. (23.59,378.27) -- (304.65,378.27) .. controls (315.32,378.27) and (323.97,386.92) .. (323.97,397.59) -- (323.97,455.55) .. controls (323.97,466.22) and (315.32,474.87) .. (304.65,474.87) -- (23.59,474.87) .. controls (12.92,474.87) and (4.27,466.22) .. (4.27,455.55) -- cycle ;
%Rounded Rect [id:dp9702560747369939] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ][line width=1.5]  (169.24,414.59) .. controls (169.24,408.28) and (174.36,403.16) .. (180.67,403.16) -- (303.81,403.16) .. controls (310.12,403.16) and (315.24,408.28) .. (315.24,414.59) -- (315.24,448.88) .. controls (315.24,455.19) and (310.12,460.31) .. (303.81,460.31) -- (180.67,460.31) .. controls (174.36,460.31) and (169.24,455.19) .. (169.24,448.88) -- cycle ;
%Straight Lines [id:da3738933457171667] 
\draw [line width=1.5]    (116.27,420.38) -- (165.24,420.38) ;
\draw [shift={(169.24,420.38)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Straight Lines [id:da13306323220327476] 
\draw [line width=1.5]    (129.65,447.38) -- (169.24,447.38) ;
\draw [shift={(125.65,447.38)}, rotate = 0] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Straight Lines [id:da33599155575798356] 
\draw [line width=1.5]    (170.48,593.51) -- (170.48,610.51) -- (308.97,610.51) -- (307.53,474.87) ;
\draw [shift={(170.48,589.51)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Straight Lines [id:da08090873505038831] 
\draw [line width=1.5]    (168.88,503.34) -- (168.88,479.34) ;
\draw [shift={(168.88,475.34)}, rotate = 450] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (13.4,-6.43) -- (0,0) -- (13.4,6.44) -- (8.9,0) -- cycle    ;
%Rounded Rect [id:dp11539642472612122] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ][line width=1.5]  (9.97,414.89) .. controls (9.97,408.49) and (15.16,403.3) .. (21.56,403.3) -- (114.06,403.3) .. controls (120.46,403.3) and (125.65,408.49) .. (125.65,414.89) -- (125.65,449.67) .. controls (125.65,456.07) and (120.46,461.26) .. (114.06,461.26) -- (21.56,461.26) .. controls (15.16,461.26) and (9.97,456.07) .. (9.97,449.67) -- cycle ;

% Text Node
\draw (243.16,415.85) node   [align=left] {\textbf{{\small System}}};
% Text Node
\draw (146.43,408.16) node  [font=\small]  {$a^{*}_{i}$};
% Text Node
\draw (151.98,457.96) node  [font=\small]  {$s_{i+1}$};
% Text Node
\draw (167.97,518.42) node   [align=left] {\textbf{{\small Heteroscedastic BO}}};
% Text Node
\draw (188.88,486.68) node  [font=\small]  {$\mathbf{x}^{*} \ $};
% Text Node
\draw (295.26,488.29) node  [font=\small]  {$g_{t\ }$};
% Text Node
\draw (169.88,554) node  [font=\small] [align=left] {$\bullet $ Set predefined noise model $\displaystyle q(\mathbf{x})$\\$\bullet $ Fit GP reward model with $\displaystyle \left(\mathbf{x}_{1:t} ,g_{1:t} ,\mathnormal{q}\right)$\\$\bullet $ Find $\displaystyle \mathbf{x}^{*}$};
% Text Node
\draw (69.05,437.26) node  [font=\small]  {$a^{*}_{i} =\text{MPC} (s_{i} ,\mathbf{x}^{*} ,f)$};
% Text Node
\draw (68.02,415.85) node   [align=left] {\textbf{Controller}};
% Text Node
\draw (243.63,437.26) node  [font=\small]  {$r_{i} =\text{SendToActuators} (a^{*}_{i} )$};
% Text Node
\draw (164.12,389.42) node   [align=left] {\textbf{Control Loop}};
\end{tikzpicture}

==> sections/figure_scripts/mpc_short.tex <==
\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-0.75,xscale=0.9]
%uncomment if require: \path (0,479); %set diagram left start at 0, and has height of 479

%Rounded Rect [id:dp25804356034521003] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ][line width=1.5]  (10.14,156.83) .. controls (10.14,152.85) and (13.37,149.62) .. (17.35,149.62) -- (188.36,149.62) .. controls (192.35,149.62) and (195.58,152.85) .. (195.58,156.83) -- (195.58,178.47) .. controls (195.58,182.46) and (192.35,185.69) .. (188.36,185.69) -- (17.35,185.69) .. controls (13.37,185.69) and (10.14,182.46) .. (10.14,178.47) -- cycle ;
%Rounded Rect [id:dp8964747104519595] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]  (248.47,157.62) .. controls (248.47,153.93) and (251.47,150.94) .. (255.16,150.94) -- (307.85,150.94) .. controls (311.55,150.94) and (314.54,153.93) .. (314.54,157.62) -- (314.54,177.68) .. controls (314.54,181.38) and (311.55,184.37) .. (307.85,184.37) -- (255.16,184.37) .. controls (251.47,184.37) and (248.47,181.38) .. (248.47,177.68) -- cycle ;
%Straight Lines [id:da14889246291929092] 
\draw [line width=1.5]    (196.35,166.95) -- (242.43,166.95) -- (244.47,166.95) ;
\draw [shift={(248.47,166.95)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (11.61,-5.58) -- (0,0) -- (11.61,5.58) -- cycle    ;
%Straight Lines [id:da518955429364597] 
\draw [line width=1.5]    (281.57,184.74) -- (281.57,205.14) -- (85.43,205.14) -- (85.39,191.01) ;
\draw [shift={(85.38,187.01)}, rotate = 449.84] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (11.61,-5.58) -- (0,0) -- (11.61,5.58) -- cycle    ;

% Text Node
\draw (102.86,167.65) node  [font=\normalsize]  {$a^{*} =\arg\min_{a\in A} \{c(s ,a)\}$};
% Text Node
\draw (281.51,167.65) node   [align=left] {\textbf{{\small System}}};
% Text Node
\draw (219.52,157.08) node  [font=\small]  {$a^{*}$};
% Text Node
\draw (187,215.27) node  [font=\small]  {$s$};


\end{tikzpicture}


==> sections/figure_scripts/scatter_plots.tex <==
\includegraphics[height=2.61cm]{images/gp_approximations/acrobot_GridS_2020_04_25__16_49_18_gridsearch_samples_norm250_homo_approximation.png}
\includegraphics[height=2.61cm]{images/gp_approximations/cartpole_GridS_2020_04_25__16_58_12_gridsearch_samples_norm250_homo_approximation.png}
\includegraphics[height=2.61cm]{images/gp_approximations/halfcheetah_GridS_2020_02_20__23_56_43_gridsearch_samples_norm250_homo_approximation.png}
\includegraphics[height=2.61cm]{images/gp_approximations/pendulum_GridS_2020_02_20__23_56_43_gridsearch_samples_norm250_homo_approximation.png}
\includegraphics[height=2.61cm]{images/gp_approximations/reacher_GridS_2020_04_25__16_58_43_gridsearch_samples_norm250_homo_approximation.png}\\
\vspace{1mm}
\includegraphics[height=2.825cm]{images/gp_approximations/acrobot_GridS_2020_04_25__16_49_18_gridsearch_samples_norm250_hetero_approximation.png}
\includegraphics[height=2.825cm]{images/gp_approximations/cartpole_GridS_2020_04_25__16_58_12_gridsearch_samples_norm250_hetero_approximation.png}
\includegraphics[height=2.825cm]{images/gp_approximations/halfcheetah_GridS_2020_02_20__23_56_43_gridsearch_samples_norm250_hetero_approximation.png}
\includegraphics[height=2.825cm]{images/gp_approximations/pendulum_GridS_2020_02_20__23_56_43_gridsearch_samples_norm250_hetero_approximation.png}
\includegraphics[height=2.825cm]{images/gp_approximations/reacher_GridS_2020_04_25__16_58_43_gridsearch_samples_norm250_hetero_approximation.png}
